Near-Optimal Streaming Ellipsoidal Rounding for General Convex Polytopes

We give near-optimal algorithms for computing an ellipsoidal rounding of a convex polytope whose vertices are given in a stream. The approximation factor is linear in the dimension (as in John's theorem) and only loses an excess logarithmic factor in the aspect ratio of the polytope. Our algorithms are nearly optimal in two senses: first, their runtimes nearly match those of the most efficient known algorithms for the offline version of the problem. Second, their approximation factors nearly match a lower bound we show against a natural class of geometric streaming algorithms. In contrast to existing works in the streaming setting that compute ellipsoidal roundings only for centrally symmetric convex polytopes, our algorithms apply to general convex polytopes. We also show how to use our algorithms to construct coresets from a stream of points that approximately preserve both the ellipsoidal rounding and the convex hull of the original set of points.

==> alg_old.tex <==
\section{Algorithm}

\begin{claim}\label{claim:vol_bound}
    Let \(t_1, \ldots, t_n \geq 0\) be such that \(\vol \cE_i \geq e^{t_i} \cdot \vol \cE_{i-1}\),
    and \(\cE_n\) satisfies \Cref{claim:alg_invariant}-(\ref{item:prop_lower}).
    Then \(\sum_{i=1}^n t_i \leq d \log\left(\frac{1}{\alpha_n}\right) + d \log\left(\frac{R}{r}\right)\).
\end{claim}
\begin{proof}
    We have \(\vol \cE_n \geq e^{\sum_{i=1}^n t_i} \vol \cE_0\),
    therefore \begin{align*}
    \sum_{i=1}^n t_i \leq \log\left(\frac{\vol(\cE_n)}{\vol(\cB_r)}\right) &= \log\left(\left(\frac{1}{\alpha_n}\right)^d\frac{\vol(\alpha_n \cdot \cE_n)}{\vol(\cB_r)}\right) \\
    &= d\log\left(\frac{1}{\alpha_n}\right) + \log\left(\frac{\vol(\alpha_n \cdot \cE_n)}{\vol(\cB_r)}\right) \\
    &\stackrel{(i)}{\leq} d\log\left(\frac{1}{\alpha_n}\right) + \log\left(\frac{\vol(\cB_R)}{\vol(\cB_r)}\right) \\
    &=d \log\left(\frac{1}{\alpha_n}\right) + d \log\left(\frac{R}{r}\right)
    \end{align*}
    where (i) follows from \(c_n + \alpha_n \cdot \cE_n \subseteq \conv{x_1, \ldots, x_n} \subseteq \cB_R\), i.e. \Cref{claim:alg_invariant}-(\ref{item:prop_lower}).
\end{proof}

\subsection{Update Step}
Consider a coordinate system where the previous ellipsoid is the unit ball centered at the origin, and the next point received is \(v = (1+s) \cdot e_1\). We can assume that \(s > 0\), as otherwise no update occurs. Let the previous ratio of inner to outer ellipsoid be \(\alpha\).
Further, let \(z^2 = x_2^2 + \ldots + x_d^2\) refer to the coordinates except \(x_1\).
The previous outer ellipsoid is defined by the equation \(x_1^2 + z^2 = 1\), and the inner ellipsoid is defined by \(x_1^2 + z^2 = \alpha^2\).

The current outer ellipsoid \(c + \cE'\) can be defined by \(A (x_1 - c)^2 + B z^2 = 1\) for \(A, B, c > 0\), with the corresponding inner ellipsoid as \(A (x_1 - c)^2 + B z^2 = \alpha'^2\) for current ratio \(\alpha'\), as shown in \Cref{fig:update_step}.
We will determine the largest value for \(\alpha'\) such that there exists a valid update with ratio \(\alpha'\).
A key observation is that this setup can be faithfully described by a two-dimensional picture: every dimension \(x_2\) through \(x_d\) behaves the same due to symmetry.


\begin{figure}[h]
\centering
\includegraphics[height=5cm]{update_step.png}
\caption{The update step.}
\label{fig:update_step}
\end{figure}

We first consider the equations that constrain the outer ellipsoid. \(\cE\) and \(c + \cE'\) must be tangent at some point, as otherwise \(\alpha'\) can be improved. Let \(\varphi \in [0, \pi/2]\) be the angle between the \(z\)-axis and the point of tangency of \(\cE\) and \(c + \cE'\), as shown in \Cref{fig:update_step_outer}.

\begin{figure}[h]
\centering
\includegraphics[height=5cm]{update_step_outer.png}
\caption{The outer ellipsoids in the update step.}
\label{fig:update_step_outer}
\end{figure}

Observe that at the point of tangency \((x, z) = (- \sin \varphi, \cos \varphi)\), the vector \((- \sin \varphi, \cos \varphi)\) defining the line \((x, z)\) is on and the gradient \((2A (x - c), 2Bz)\) of the equation defining the ellipsoid \(c + \cE'\) must be parallel. 
Thus \(B z x = A z(x-c)\), i.e.
\begin{equation}\label{eqn:outer_1}
    A (\sin \varphi + c) = B \sin \varphi
\end{equation}
As the point of tangency must be on \(c + \cE'\), we also have
\begin{equation}\label{eqn:outer_2}
    A (\sin \varphi + c)^2 + B \cos^2 \varphi = 1
\end{equation}
Finally, \((1+s, 0)\) must be on \(c + \cE'\) as well, so
\begin{equation}\label{eqn:outer_3}
    A (1+s - c)^2 = 1
\end{equation}

Solving these equations (\ref{eqn:outer_1}), (\ref{eqn:outer_2}), (\ref{eqn:outer_3}) for \(A, B, c\) in terms of \(s\) and \(\varphi\), we get:
% Older equations
% \begin{equation}
%     A = \frac{1}{\left(\Delta t-\frac{2 (-1 + {\Delta t}^2) \sin(\varphi)}{3 + 4 \Delta t \sin(\varphi) - \cos(2\varphi)}\right)^2}, \quad
%     B = \frac{3 + 4 \Delta t \sin(\varphi) - \cos(2\varphi)}{2 (1 + \Delta t \sin(\varphi))^2}, \quad
%     c = \frac{2 (-1 + {\Delta t}^2) \sin(\varphi)}{3 + 4 \Delta t \sin(\varphi) - \cos(2\varphi)}
% \end{equation}
\begin{equation}\label{eqn:outer_params}
\left.\begin{aligned}
    A = A^0(s, \varphi) &\defeq \frac{(\cos^2(\varphi)+2\sin(\varphi)(1+s + \sin(\varphi))^2}{(1+s + \sin(\varphi))^2(1+(1+s) \sin(\varphi))^2} \\
    B = B^0(s, \varphi) &\defeq \frac{1 + \sin^2(\varphi) + 2(1+s) \sin(\varphi)}{(1+(1+s) \sin(\varphi))^2}\\
    c = c^0(s, \varphi) &\defeq \frac{s(2+s)\sin(\varphi)}{1 + \sin^2(\varphi) + 2(1+s) \sin(\varphi)}
\end{aligned}\qquad
\right\}
\end{equation}
In summary, this gives a formula for the update \(c + \cE'\) in terms of \(s\) and \(\varphi\).
However, we have not yet considered how \(\alpha'\) is constrained.

Thus, we consider the equations that constrain the inner ellipsoid.
Let \(L\) be the line tangent to the previous inner ellipsoid \(\alpha \cE\) that goes through \(v\),
and let \((\hat{x}, \hat{z})\) be the point of tangency between \(L\) and \(\alpha \cE\).
Let \((x', z')\) be the point on \(c + \alpha' \cE'\) where the tangent line is parallel to \(L\).
This is illustrated in \Cref{fig:update_step_inner}.

\begin{figure}[h]
\centering
\includegraphics[height=5cm]{update_step_inner.png}
\caption{The inner ellipsoids in the update step.}
\label{fig:update_step_inner}
\end{figure}

We determine the equation defining \(L\). As the normal vector of \(L\) is parallel to \((\hat{x}, \hat{z})\), we can write it as \(\hat{x} x + \hat{z} z = \alpha^2\).
As \(v\) lies on \(L\), we have \(\hat{x} (1+s) = \alpha^2\) so \(\hat{x} = \frac{\alpha^2}{1+s}\).
Because \(\hat{x}^2 + \hat{z}^2 = \alpha^2\), we have \(\hat{z} = \sqrt{\alpha^2 - \frac{\alpha^4}{(1+s)^2}} = \alpha \sqrt{1 - \frac{\alpha^2}{(1+s)^2}}\).
By dividing all sides by \(\alpha^2\), we can also write the equation of \(L\) as \(\frac{x}{1+s} + z \sqrt{\frac{1}{\alpha^2} - \frac{1}{(1+s)^2}} = 1\).

The length of the major semi-axis (along \(x_1\)) of the current outer ellipsoid \(c + \cE'\) is \(1/\sqrt{A}\) by definition, so the length of the same axis of the inner ellipsoid is \(\alpha'/\sqrt{A}\).
As the leftmost point of \(c + \alpha' \cE'\) must be contained within \(\alpha \cE\), and it lies on the same axis as \((-\alpha, 0)\), we must have
\(c - \frac{\alpha'}{\sqrt{A}} \geq -\alpha\), so
\begin{equation}\label{eqn:inner_approx_1}
   \alpha' \leq \alpha^1(s, \varphi, \alpha) \defeq (\alpha + c) \sqrt{A}
\end{equation}

\((x', z')\) is defined by being on the inner ellipsoid, with its tangent parallel to \(L\).
The gradient of the equation defining \(c + \alpha' \cE'\) at \((x', z')\) is \((2 A (x' - c), 2 B z')\), which means
we have
\begin{equation}\label{eqn:inner_conv_1}
    A (x' - c) \sqrt{\frac{1}{\alpha^2}-\frac{1}{(1+s)^2}} = \frac{1}{1+s} B z'
\end{equation}
Because \((x', z')\) lies on the inner ellipsoid \(c + \alpha' \cE'\), we have
\begin{equation}\label{eqn:inner_conv_2}
    A (x' - c)^2 + B z'^2 = \alpha'^2
\end{equation}
Finally, \(c+ \alpha' \cE'\) must be contained within \(\conv{\alpha \cE \cup \{v\}}\), which implies that \((x', z')\) must be at least as close to the origin as \(L\). This gives
\begin{equation}\label{eqn:inner_conv_3}
    \frac{x'}{(1+s)} + \sqrt{\frac{1}{\alpha^2} - \frac{1}{(1+s)^2}} \cdot z' \leq 1
\end{equation}

The equation (\ref{eqn:inner_approx_1}) gives an upper bound on \(\alpha'\) using the leftmost point of \(\conv{\alpha \cE \cup \{v\}}\), so now we use (\ref{eqn:inner_conv_1}), (\ref{eqn:inner_conv_2}), (\ref{eqn:inner_conv_3}) to give another upper bound on \(\alpha'\) using \(L\).
Consider the smallest \(\alpha''\) such that \(c + \alpha'' \cE'\) touches \(L\), clearly \(\alpha'' \geq \alpha'\). If we define \((x', z')\) to lie on this ellipsoid \(c + \alpha'' \cE'\) instead, then (\ref{eqn:inner_conv_1}) is unchanged, (\ref{eqn:inner_conv_3}) becomes an equality,
and for (\ref{eqn:inner_conv_2}) we get \(\alpha''= A (x' - c)^2 + B z'^2 \geq \alpha'^2\).
The advantage of this rewrite is that now (\ref{eqn:inner_conv_1}) and (\ref{eqn:inner_conv_3}) form a linear system in \((x', z')\).
Solving this linear system, we get
\[
x' = \frac{(s+1) \left(A c (s+1) \sqrt{1-\frac{\alpha ^2}{(s+1)^2}} \sqrt{\frac{1}{\alpha ^2}-\frac{1}{s+1}}+\alpha  B\right)}{A (s+1)^2 \sqrt{1-\frac{\alpha ^2}{(s+1)^2}} \sqrt{\frac{1}{\alpha ^2}-\frac{1}{s+1}}+\alpha  B}, \quad
z' = \frac{\alpha  A (s+1) (-c+s+1) \sqrt{\frac{1}{\alpha ^2}-\frac{1}{s+1}}}{A (s+1)^2 \sqrt{1-\frac{\alpha ^2}{(s+1)^2}} \sqrt{\frac{1}{\alpha ^2}-\frac{1}{s+1}}+\alpha  B}
\]

Using this solution in (\ref{eqn:inner_conv_2}), we get our second upper bound on \(\alpha'\) in addition to (\ref{eqn:inner_approx_1}):
\begin{equation}\label{eqn:inner_approx_2}
    \alpha' \leq \alpha^2(s, \varphi, \alpha) \defeq \sqrt{\frac{A B (-c+s+1)^2 \left(A (s+1) \left(-\alpha ^2+s+1\right)+\alpha ^2 B\right)}{\left(A (s+1)^2 \sqrt{1-\frac{\alpha ^2}{(s+1)^2}} \sqrt{\frac{1}{\alpha ^2}-\frac{1}{s+1}}+\alpha  B\right)^2}}
\end{equation}

Thus the best possible \(\alpha'\) is the minimum of these two upper bounds:
\begin{equation}\label{eqn:inner_approx_param}
    \alpha^{0}(s, \varphi, \alpha) \defeq \min(\alpha^1(s, \varphi, \alpha), \alpha^2(s, \varphi, \alpha))
\end{equation}

\subsection{Continuous Update}

Now, we will define a continuous-time process that will evolve the ellipsoids \(c + \cE', c + \alpha' \cE'\) according to instantaneous versions of the update equations from the previous section. The equations from the previous section describe the update to the unit ball after adding the point \(((1+s), 0)\). We will now take \(s\) to be very small, and repeatedly add a point `just outside' the current outer ellipsoid.

In particular, let \(A(t), B(t), c(t), \alpha(t) \colon \R_{\geq 0} \to \R\) be functions describing the current outer and inner ellipsoids 
\[\underbrace{A(t) \cdot (x_1 - c(t))^2 + B(t) z^2 = 1}_{c(t) + \cE(t)}, \qquad \underbrace{A(t)\cdot (x_1 - c(t))^2 + B(t) z^2 = \alpha(t)^2}_{c(t) + \alpha(t) \cE(t)}\]
We will let \(\alpha^0\) be\maxcmt{overloads with \(\alpha^0\) the function from (\ref{eqn:inner_approx_param}). may need to change this} the previous approximation factor, so that
the starting configuration is \(c(0) + \cE(0) = B_2^d, c(0) + \alpha(0) \cE(0) = \alpha^0 B_2^d\) with initial conditions \(A(t) = 1, B(t) = 1, c(t) = 0, \alpha(t) = \alpha^0\).
While the equations from the previous section can describe the instantaneous update at time \(t = 0\), they only describe the update when the previous ellipsoid is the unit ball centered at 0.
For a time \(t_0 \geq 0\), we therefore consider the affine transformation \(F_{t_0} \colon \R^2 \to \R^2\)
\[(x, z) \mapsto \inparen{ c(t_0) + x/\sqrt{A(t_0)}, z/\sqrt{B(t_0)}}\]

For any \(t_0\), observe that this transformation maps the unit ball centered at zero \(B_2^d\) to the ellipsoid \(c(t_0) + \cE(t_0)\), as the axes of \(c(t_0) + \cE(t_0)\) have lengths \(1/\sqrt{A(t_0)}, 1/\sqrt{B(t_0)}\).
At \(t_0 = 0\) this transformation is the identity, consistent with the previous section.

In this coordinate system, the equations describing \(c(t) + \cE(t), c(t) + \alpha(t)\cE(t)\) can be written as
\[\frac{A(t)}{A(t_0)} \inparen{x - \sqrt{A(t_0)}(c(t) - c(t_0))}^2 + \frac{B(t)}{B(t_0)} z^2 = 1, \quad \frac{A(t)}{A(t_0)} \inparen{x - \sqrt{A(t_0)}(c(t) - c(t_0))}^2 + \frac{B(t)}{B(t_0)} z^2 = \alpha(t)^2 \]

Therefore, updating with point \(v = ((1+s), 0)\) (written in this coordinate system) and recalling (\ref{eqn:outer_params}), (\ref{eqn:inner_approx_param}) yields equations
\[\frac{A}{A(t_0)} = A^0(s, \varphi), \ \frac{B}{B(t_0)} = B^0(s, \varphi), \ \sqrt{A(t_0)}(c-c(t_0)) = c^0(s, \varphi), \ \alpha = \alpha^0(s, \varphi, \alpha)\]

To describe the instantaneous update at time \(t_0\), we take the derivative with respect to \(s\) at \(s = 0\).
Thus for all \(t\), we obtain the differential equations
\begin{equation}\label{eqn:update_ode}
\left.\begin{aligned}
\frac{d A(t)}{dt} &= A(t) \cdot \left.\frac{\partial A^0(s, \varphi)}{\partial s}\right|_{s=0} \\
\frac{d B(t)}{dt} &= B(t) \cdot \left.\frac{\partial B^0(s, \varphi)}{\partial s}\right|_{s=0} \\
\frac{d c(t)}{dt} &= \sqrt{A(t)} \cdot \left.\frac{\partial c^0(s, \varphi)}{\partial s}\right|_{s=0} \\
\frac{d \alpha(t)}{dt} &= \left.\frac{\partial \alpha^0(s, \varphi, \alpha(t))}{\partial s}\right|_{s=0}
\end{aligned}
\right\}
\end{equation}

Clearly, these equations depend on the choice of \(\varphi\), which may also evolve with time.
In the analysis, we will see that the choice \(\varphi = \frac{1}{2} \alpha (1 - \alpha)\) will eventually lead to a good approximation factor.

\subsection{Analysis of Continuous Update}

\(\alpha(t)\) describes the approximation factor of the process with time, and in order to bound the approximation factor we would like to
analyze this quantity. However, it is difficult to obtain an analytical solution to the differential equation in (\ref{eqn:update_ode}). Therefore, our strategy is to lower bound \(\frac{d\alpha(t)}{dt}\), and use the differential equation for this lower bound instead.

Let \(\alpha'(s, \alpha) =\alpha^0(s, \frac{1}{2} \alpha (1-\alpha), \alpha)\), i.e. the bound (\ref{eqn:inner_approx_param}) using the choice \(\varphi = \frac{1}{2} \alpha (1-\alpha)\). We give the following lower bound on the approximation factor for the update step:

\begin{claim}\label{claim:bound_alpha_derivative}
    There exists \(c > 0\) for which \(\alpha'(s, \alpha) - \alpha \geq - c \alpha^2 \cdot s + \cO(s^2)\).
\end{claim}

It turns out that \(c = 1\), which is shown in \Cref{claim:proof_bound_alpha_derivative}.

\begin{proof}
    We examine the Taylor series \(\alpha'(s, \alpha) - \alpha = c_0 + c_1 s + O(s^2)\).
    We have that \(\alpha'(0, \alpha) = \alpha\), so \(c_0 = 0\).
    \maxcmt{I don't see a way to do this that isn't just a less sophisticated version of the proof in \Cref{claim:proof_bound_alpha_derivative}. Still need to take the derivative with respect to \(s\) analytically, I think?}
\end{proof}

Now, we use this to bound \(\alpha(t)\).
\begin{claim}
    Let \(\alpha(t)\) be a solution to (\ref{eqn:update_ode}) with initial condition \(\alpha(0) = \alpha^0\).
    Then for all \(t \geq 0\),
    \[\frac{1}{\alpha(t)} \leq t + \frac{1}{\alpha^0}\]
\end{claim}
\begin{proof}
We compare \(\alpha(t)\) with the solution of another differential equation via a differential inequality.
First, we have by definition (\ref{eqn:update_ode}) that \(\frac{d \alpha(t)}{dt} = \left.\frac{\partial \alpha'}{\partial s}\right|_{s = 0}\).
Observe that by dividing both sides of \Cref{claim:bound_alpha_derivative} by \(s\) and taking \(s \to 0\), we get
\[
\left.\frac{\partial \alpha'}{\partial s}\right|_{s = 0} \geq - \alpha^2
\]
Thus we consider the differential equation
\[
\frac{d \beta}{dt} = - \beta^2 
\]
with initial condition \(\beta(0) = \alpha^0\).
This is a well-known separable ODE, with solution \(\frac{1}{\beta(t)} = t + \mathsf{Const}\). Using the initial condition we obtain the solution
\(\frac{1}{\beta(t)} = t + \frac{1}{\alpha^0}\). As the derivative \(\frac{d \beta}{dt}\) is \(C^1\), by \Cref{thm:diffe_unique_cont} the solution is unique.
Then by \Cref{thm:diffe_ineq}, we have \(\alpha(t) \geq \beta(t)\) for all \(t \geq 0\), and therefore
\(\frac{1}{\alpha(t)} \leq t + \frac{1}{\alpha^0}\).
\end{proof}

\begin{definition}
    \((c' + \cE', \alpha')\) is a valid next step\maxcmt{Open to other names for this} for \((c + \cE, \alpha, v)\) if
    \begin{enumerate}
        \item \(\conv{c' + \cE' \cup \{v\}} \subseteq c +\cE\)
        \item \(c' + \alpha' \cE' \subseteq \conv{\alpha \cE \cup \{v\}}\)
    \end{enumerate}
\end{definition}

Let \(t^* = 2 \log(\|v_i - c_i\|_{\cE_{i-1}})\). Then \(t^* \leq 2 (\log\vol \cE_{i} - \log \vol \cE_{i-1})\).

\begin{claim}\label{claim:cont_valid}
    \((c(t^*) + \cE(t^*), \alpha(t^*))\) is a valid next step for \((c + \cE, \alpha, v)\).
\end{claim}

\begin{claim}\label{claim:cont_approx}
We have
\[\frac{1}{\alpha(t^*)} - \frac{1}{\alpha_0} \leq \log \vol(\cE_{i+1}) - \log\vol(\cE_i)\]
\end{claim}

We will denote 

\subsection{Algorithm}

Implementation given in \Cref{alg:main}.

\begin{algorithm}
\caption{Streaming Ellipsoidal Approximation}\label{alg:main}
  \begin{algorithmic}[1]
    \State Initialize \(c_0 = 0, \cE_0 = B_r, \alpha_0 = 1\)
    \For{\(i = 1, \ldots, n\)}
      \State Receive \(v_i\)
      \If{\(\|v_i - c_i\|_{\cE_{i-1}} > 1\)}
        \State \(\alpha_i = \) the largest \(\alpha\) for which there exists a valid next step \((c', \cE', \alpha)\) for \((c_{i-1} + \cE_{i-1}, \alpha_{i-1}, v_i)\) \label{alg_line:main_findapprox}
      \Else
        \State \(c_i = c_{i-1}, \cE_i = \cE_{i-1}\)
      \EndIf
    \EndFor
  \end{algorithmic}
\end{algorithm}

Though Line~\ref{alg_line:main_findapprox} in this algorithm is unambiguous, it may not be immediately clear how to implement it efficiently.

\begin{claim}
    For all \(1 \leq i \leq n\):
    \[\frac{1}{\alpha_{i}} - \frac{1}{\alpha_{i-1}} \leq \log \vol(\cE_{i}) - \log\vol(\cE_{i-1})\]
\end{claim}
\begin{proof}
    By definition, \(\alpha_i \)
\end{proof}

\section{Appendix}

\section{Details of Algorithm Analysis}
In this section we prove \Cref{claim:bound_alpha_derivative} and show that the constant \(c= 1\).
\begin{proof}[Proof of \Cref{claim:bound_alpha_derivative}]\label{claim:proof_bound_alpha_derivative}
Let \(U_1(s, \alpha) = \alpha^1\inparen{s, \frac{\alpha(1-\alpha)}{2}, \alpha}\) and \(U_2(s, \alpha) = \alpha^2\inparen{s, \frac{\alpha(1-\alpha)}{2}, \alpha}\), recalling the expressions (\ref{eqn:inner_approx_1}) and (\ref{eqn:inner_approx_2}) respectively.
\(\varphi = \frac{\alpha(1-\alpha)}{2}\) is chosen to maximize the lower bound on \(\alpha'(s, \alpha)\).
Recall that \(\alpha'(s, \alpha) = \min(U_1(s, \alpha), U_2(s, \alpha))\). In order to bound \(\alpha'\) from below, we examine the Taylor series of \(U_1\) and \(U_2\) around \(s = 0\).

First, observe that \(U_1(0, \alpha) = U_2(0, \alpha) = \alpha\).
Taking the partial derivatives at \(s = 0\) and simplifying, we get:
\[
\left.\frac{\partial U_1(s, \alpha)}{\partial s}\right|_{s=0}=\frac{-3 \alpha -4 \sin \left(\frac{1}{2} (\alpha -1) \alpha \right)+\alpha  \cos ((\alpha -1) \alpha )}{2 \left(\sin \left(\frac{1}{4} (1-\alpha ) \alpha \right)+\cos \left(\frac{1}{4} (\alpha -1) \alpha \right)\right)^4}
\]
\[
\left.\frac{\partial U_2(s, \alpha)}{\partial s}\right|_{s=0} = \frac{\alpha  \left(-2 \alpha ^2+4 \sin \left(\frac{1}{2} (\alpha -1) \alpha \right)+\cos ((\alpha -1) \alpha )-1\right)}{2 \left(\sin \left(\frac{1}{4} (1-\alpha ) \alpha \right)+\cos \left(\frac{1}{4} (\alpha -1) \alpha \right)\right)^4}
\]

Now, to show \(\alpha'(s, \alpha) - \alpha \geq - \alpha^2 s + \cO(s^2)\), it suffices to show that \(\left.\frac{\partial U_1(s, \alpha)}{\partial s}\right|_{s=0} \geq - \alpha^2\) and \(\left.\frac{\partial U_2(s, \alpha)}{\partial s}\right|_{s=0} \geq - \alpha^2\).
This can be seen in \Cref{fig:apdx_derivative_bounds}.
\begin{figure}[h]
\centering
\includegraphics[height=4cm]{series_plot.png}
\caption{Plot of \(\frac{1}{\alpha^2} \cdot \left[\frac{\partial U_1(s, \alpha)}{\partial s}\right]_{s=0}, \quad \frac{1}{\alpha^2} \cdot \left[\frac{\partial U_2(s, \alpha)}{\partial s}\right]_{s=0}\) versus \(-1\)}
\label{fig:apdx_derivative_bounds}
\end{figure}
\end{proof}

\section{Background on Differential Equations}
We briefly review some of the relevant background on ordinary differential equations, see e.g. \cite{hale2009ordinary}.
Let \(U(t,u) \colon E \to \R\) be a continuous function on an open connected set \(E \subseteq \R^2\). We consider solutions to the initial value problem
\begin{equation}\label{eqn:diffe_ivp}
    \frac{du}{dt} = U(t,u), \quad u(a) = u_0
\end{equation}
for \((a, u_0) \in E\).

We say that \(U\) is locally Lipschitz with respect to \(u\) on \(E\) if for every closed and bounded \(S \subseteq E\), there is an \(L_S > 0\) such that \(|U(t,u) - U(t,v)| \leq L_S |u - v|\) for all \((t, u), (t, v) \in S\).
In this case, unique solutions to (\ref{eqn:diffe_ivp}) exist:

\begin{theorem}[Theorem 3.1, Section 1.3 of \cite{hale2009ordinary}]\label{thm:diffe_unique}
If \(U(t,u)\) is locally Lipschitz with respect to \(u\), then there exists a unique solution to (\ref{eqn:diffe_ivp}).
\end{theorem}

As a continuous first derivative is sufficient for local Lipschitzness, we get the following:
\begin{corollary}\label{thm:diffe_unique_cont}
If \(\frac{\partial U(t,u)}{\partial u}\) is continuous with respect to \(u\) in \(E\), then \(U\) is locally Lipschitz with respect to \(u\) in \(E\), and there exists a unique solution to (\ref{eqn:diffe_ivp}).
\end{corollary}

Finding the analytical solution for some differential equations in this paper is difficult,
so we instead use the method of differential inequalities to bound solutions.
We say a \(v(t) \colon [a,b] \to \R\) is a solution of the differential inequality 
\begin{equation}\label{eqn:diffe_ineq}
\frac{dv}{dt} \leq U(t,v(t))
\end{equation} if it is differentiable on \([a, b]\) and satisfies the inequality for all \(t \in [a,b]\).

\begin{theorem}[Theorem 6.1, Section 1.6 of \cite{hale2009ordinary}]\label{thm:diffe_ineq}
Let \(I = [a,b]\) be an interval. If (\ref{eqn:diffe_ivp}) has a unique solution \(u\) on \(I\), and \(v\) is a solution of (\ref{eqn:diffe_ineq}) on \(I\) such that \(v(a) \leq u(a)\), then \(v \leq u\) on \(I\).
\end{theorem}



==> aspect_ratio_vs_n.tex <==
\section{Aspect ratio of polytopes}

In this section, we prove Lemma \ref{lemma:aspect_ratio_vs_n}.

\begin{lemma}
\label{lemma:aspect_ratio_vs_n}
Let $P \subset \R^d$ be a polytope with $n$ vertices and let $r, R$ be the largest and smallest values, respectively, such that
\begin{align*}
    r \cdot B_2^d \subseteq P \subseteq R \cdot B_2^d.
\end{align*}
There exists a universal constant $C$ such that $\nfrac{R}{r} \ge \inparen{\frac{d}{C \log n}}^{C}$.
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lemma:aspect_ratio_vs_n}]
We proceed through a volume argument. Without loss of generality, let $R = 1$. Our task is to bound $\nfrac{1}{r}$. It is well-known (see, e.g., Exercise 7.4.5 due to \citet{vershynin_2018}, the proof of which follows from Sudakov's inequality) that
\begin{align*}
    \frac{\mathsf{Vol}(P)}{\mathsf{Vol}(B_2^d)} \le \inparen{\frac{C \log n}{d}}^{Cd}.
\end{align*}
Let $r$ be some value for which $r \cdot B_2^d \subseteq P$. Notice that we have
\begin{align*}
    r^d = \frac{\mathsf{Vol}(r \cdot B_2^d)}{\mathsf{Vol}(B_2^d)} \le \frac{\mathsf{Vol}(P)}{\mathsf{Vol}(B_2^d)} \le \inparen{\frac{C \log n}{d}}^{Cd}
\end{align*}
which implies
\begin{align*}
    \frac{1}{r} \ge \inparen{\frac{d}{C\log n}}^{C}.
\end{align*}
This concludes the proof of Lemma \ref{lemma:aspect_ratio_vs_n}.
\end{proof}

==> irregular.tex <==

\section{Irregular Update Step}
We consider the irregular update step of the algorithm for computing a core set.

As discussed, we need to analyze the following problem. Find an ellipse $\cal E = \{(x,y): Ax^2 + By^2 \leq 1\}$, point $(0,c)$ and a parameter $\tilde \alpha$ so as to maximize $\hat \alpha$ so that
\begin{itemize}
\item Ellipse $(0,c) + \cal E = \{(x,y): Ax^2 + B(y-c)^2 \leq 1\}$ contains points $(\pm 1, 0)$ and $(0,1)$; that is,
\[A +B c^2 \leq 1\qquad\text{and}\qquad
B(1-c)^2 \leq 1
\]
\item The inner ellipse $(0,c) + \tilde\alpha{\cal E}$ lies inside the triangle with vertices $(0,1), (-\alpha, 0), (\alpha, 0)$. That is, $(0,0)$ lies outside of $(0,c) + \tilde\alpha{\cal E}$:
\[
Bc^2 \geq \tilde\alpha^2
\]
and the line through points $(0,1)$ and $(\alpha,0)$ lies outside of the ellipse:
\[
\tilde \alpha \leq (1-c) \frac{\sqrt{AB}}{\sqrt{A\alpha^2 +B}}\alpha
\]
\end{itemize}
It is easy to see that the latter upper bound increases when $A$ increases, thus $A = 1-Bc^2$ in the optimal solution. We get,
\begin{align*}
    \text{\bf maximize } & \min\left(\sqrt{B} c, (1-c)\sqrt{\frac{B(1-Bc^2)}{B + (1-B c^2) \alpha^2}} \cdot \alpha\right)\\
    \text{\bf s.t. } & B(1-c^2) \leq 1\\
    &Bc^2 \leq 1
\end{align*}
We are interested in the regime where $c^2 \ll 1/2$ and thus the second inequality is not tight (and the first one is likely tight).

For a feasible solution given by $B = \frac{1}{1-c^2}$ and $c=\alpha$, we get
$\tilde \alpha = \alpha - \alpha^3 - O(\alpha^4)$.



==> main_leverage_connection.tex <==

\section{Connections to Online Leverage-Score Based Algorithms}
although as described in the introduction unclear how to do recentering procedure to use leverage scores to solve
our, here we describe a connection between previous work that and work that uses leverage scores in the symmetric case
\cite{mmo22}
online here, connect to ellipsoid online
\maxcmt{Still missing context and how to frame this}

We first restate in \Cref{alg:wy22} the online \(\ell_\infty\) subspace sketch coreset from \cite{woodruff2022high},
in a notation that more closely matches ours.
\begin{algorithm}[h]
\caption{Online \(\ell_\infty\) Subspace Sketch Coreset, Algorithm 1 from \cite{woodruff2022high}}\label{alg:wy22}
\textbf{input}: \(\vz_1, \ldots, \vz_n \in \R^{d}\) \\
\textbf{output}: Coreset \(S \subseteq [n]\)
\begin{algorithmic}[1]
\State \(S \leftarrow \varnothing\)
\For{\(i \in [n]\)}
    \If{\(\exists \vx \in \R^n \colon \langle \vz_i, \vx \rangle^2 \geq \|\mZ|_S \vx\|_2^2\)}
        \State \(S \leftarrow S \cup \{i\}\)
    \EndIf{}
\EndFor
\State \Return \(S\)
\end{algorithmic}
\end{algorithm}

By \(\mZ|_S\) we mean the matrix whose rows are \(\{\vz_i\}_{i \in S}\).

talk about leverage scores, interpretation for certain ellipsoid

real entries, our setting is closer to their online coreset model as opposed to the integer entries
\[\mZ\vert_S^\top \mZ\vert_S = \sum_{i \in S} \vz_i \vz_i^\top\]
Let \(\mA \in \R^{d \times d}\) be such that \(\mZ^\top \mZ = (\mZ\vert_S^\top \mZ\vert_S)^{-}\), for example by \(\mA = \inparen{(\mZ\vert_S^\top \mZ\vert_S)^{-}}^{1/2}\). Rewrite update \(\vz_i^\top (\mZ\vert_S^\top \mZ\vert_S)^- \vz_i > 1\) if and only if \(\vz_i \not\in \cE_{\mA}\).

\cite{mmo22}, Claim 8. symmetric update rule \(\cU(\cE, \vz)\). Updates if and only if \(\vz \not\in \cE\). Given an ellipsoid \(\cE_{\mA}\) and a point \(\vz \not\in \cE\),
updates \(\mA' = \hat{\mA} \mA\), where
\begin{equation}
\hat{\mA} = \mI_d - \left(1 - \frac{1}{\|\mA \vz\|}\right) \frac{(\mA \vz) (\mA \vz)^\top}{\|\mA \vz\|^2}
\end{equation}

Assume that \(\mB^{-1} = \mA^\top \mA\).
We have \(\mA' = \widehat{\mA} \cdot \mA\) where \(\vy_i = \sqrt{1 + \frac{1}{\|\mA_{i-1} \vv_i\|^2}} \cdot \vv_i\).
Like giving the update \(\cU(\cE_{\mA_{i-1}}, \vy_i)\)
\maxcmt{have some connection to the coreset algorithm we design - scaled version. could be helpful interpretation}
\[\hat{\mA}_i = \mI_d - \left(1 - \frac{1}{\|\mA_{i-1} \vy_i\|}\right) \frac{(\mA_{i-1} \vy_i) (\mA_{i-1} \vy_i)^\top}{\|\mA_{i-1} \vy_i\|^2}\]
\begin{lemma}
\[(\mB + \vz \vz^\top)^{-1} = \mA'^\top \mA'\]
\end{lemma}
\begin{proof}
Let \(\vw = \frac{\mA\vy}{\|\mA \vy\|}\) be a unit vector, and let \(\mW \in \R^{d \times d}\)
be a orthogonal matrix with \(\vw\) as its first column.
Observe that we can write
\[\hat{\mA} = \mW \cdot \diag{\frac{1}{\|\mA \vy\|}, 1, \ldots, 1} \cdot \mW^\top\]
Taking the square, this means
\begin{align*}
    \widehat{\mA}^2 &= \mW \cdot \diag{\frac{1}{\|\mA \vy\|^2}, 1, \ldots, 1} \cdot \mW^\top \\
    &= \mI_{d} - \left(1 - \frac{1}{\|\mA \vy\|^2}\right) \frac{(\mA \vy) (\mA \vy)^\top}{\|\mA \vy\|^2}
    % &= \mI_{d} - \left(1 - \frac{1}{\left(1 + \frac{1}{\|A v\|^2}\right) \|A v\|^2}\right) \frac{(Av) (Av)^\top}{\|Av\|^2} \\
    % &= \mI_d - \frac{1}{1 + \|Av\|^2} (Av) (Av)^\top
\end{align*}
Plugging in the definition of \(\vy\), we get the formula
\begin{equation}\label{eqn:cc_square_hat_a}
\hat{\mA}^2 = \mI_d - \frac{1}{1 + \|\mA \vz\|^2} (\mA \vz) (\mA \vz)^\top
\end{equation}
Sherman-Morrison formula \cite{sherman1950adjustment} gives
\[(\mB + \vz \vz^\top)^{-1} = \mB^{-1} - \frac{\mB^{-1} \vz \vz^\top \mB^{-1}}{1 + \vz^\top \mB^{-1} \vz}\]
Using \(\mB^{-1} = \mA^\top \mA\), we have
\begin{align*}
    (\mB + \vz \vz^\top)^{-1} &= \mA^\top \left(\mI_d - \frac{\mA \vz \vz^\top \mA^\top}{1 + \|\mA \vz\|^2}\right) \mA \\
    &= \mA^\top \hat{\mA}^2 \mA & \text{by (\ref{eqn:cc_square_hat_a})} \\
    &= \mA'^\top \mA'
\end{align*}
as desired.
\end{proof}

Can interpret leverage scores as alternate way to `regularize' updates, by ensuring norm is at least
\[\|\mA_{i-1} \vy_i\| = \sqrt{1 + \frac{1}{\|\mA_{i-1} \vv_i\|^2}} \cdot \| \mA_{i-1} \vv_i \| = \sqrt{1 +\|\mA_{i-1} \vv_i\|^2} \geq \sqrt{2}\]
as the update only happens in the first place when \(\|\mA_{i-1} \vv_i\| > 1\).

compare to our coreset that only updates when the volume increases

% \maxcmt{general is pseudo-inverses, need to understand this still.
% There is a Sherman-Morrison formula for pseudoinverses at \url{https://epubs.siam.org/doi/pdf/10.1137/0124033}}


==> main_select_vertices_symmetric.tex <==
In this subsection, we improve the construction of the core-set when the convex body in question is symmetric. The main result of this subsection is Theorem \ref{thm:online_coreset_symmetric}.

% In this subsection, we describe an extension of our techniques to the setting studied in \cite{woodruff2022high}.

% First, we restate the main problem studied in \cite{woodruff2022high}.

% \begin{problem}[Streaming $\linf$ subspace sketching -- See Definition 1.1 of \cite{woodruff2022high}]
% \label{problem:subspace_sketching}
% In what follows, for a matrix $X \in \R^{n\times d}$ and a subset $S \subseteq [n]$, let $X\vert_S$ be the matrix obtained by restricting $X$ to the rows indexed by $S$.

% Let $X \in \R^{n\times d}$ be a matrix given to us in a row arrival stream. Then:
% \begin{itemize}
%     \item In the \emph{row arrival streaming model}, let $X \in \Z^{n\times d}$ have entries bounded by $\mathsf{poly}(n)$. We must maintain a data structure $\myfunc{Q}{\R^d}{\R}$ such that, at the end of the stream, we have for some $\alpha \ge 1$ that:
%     \begin{align*}
%         \text{for all } y \in \R^d, \maxnorm{Xy} \le Q(y) \le \alpha \cdot \maxnorm{Xy}
%     \end{align*}
%     \item In the \emph{online coreset model}, let $X \in \R^{n \times d}$ be a real matrix. We must irrevocably choose a subset of entries $S \subseteq [n]$ and weights $w \in \R^S$ as well as a function $\myfunc{Q}{\R^d}{\R}$ depending only on $\diag{w}X\vert_S$ such that, at the end of the stream, we have for some $\alpha \ge 1$ that:
%     \begin{align*}
%         \text{for all } x \in \R^d, \maxnorm{Xy} \le Q(y) \le \alpha \cdot \maxnorm{Xy}
%     \end{align*}
% \end{itemize}
% \end{problem}

% The authors of \cite{woodruff2022high} give algorithmic results for Problem \ref{problem:subspace_sketching} (see Theorem \ref{thm:subspace_sketching}). They use this as a meta-approach to give algorithms for a variety of streaming linear algebra and streaming computational geometry tasks, including convex hull sketching, streaming ellipsoidal approximations\footnote{The approximation factor given in \cite{woodruff2022high} for streaming ellipsoidal approximations is suboptimal by a factor of $\Omega\inparen{\sqrt{d}}$; see Theorem 1.10.}, $k$-robust directional width, $\ell_p$ subspace sketch for $p < \infty$, volume maximization, minimum-width spherical shell, and solving linear programs. See Section 1.1 of \cite{woodruff2022high} for more details.

% \begin{theorem}[See Theorem 1.3 of \cite{woodruff2022high}]
% \label{thm:subspace_sketching}
% Let $\kappaol$ be the \emph{online condition number} of $X$ -- that is, $\kappaol(X) \coloneqq \opnorm{X} \cdot \max_{i \in [n]} \opnorm{X\vert_{[i]}^{+}}$, where $X^{+}$ denotes the Moore-Penrose pseudoinverse of $X$.

% Let $X \in \R^{n \times d}$ be presented in one pass over a row arrival stream. There is an algorithm $\cA$ which maintains a coreset $S \subseteq [n]$ such that:
% \begin{align*}
%     \text{for all } y \in \R^d, \maxnorm{X\vert_S \cdot y} \le \maxnorm{Xy} \le \alpha \cdot \maxnorm{X\vert_S \cdot y}
% \end{align*}
% where:
% \begin{itemize}
%     \item in the row arrival streaming model, $\alpha = O\inparen{\sqrt{d \log n}}$, $\abs{S} = O(d \log n)$, and $\cA$ uses $O(d^2 \log^2 n)$ bits of space.
%     \item in the online coreset model, $\alpha = O\inparen{\sqrt{d\log \kappaol(X)}}$ and $\abs{S} = O\inparen{d \log \kappaol(X)}$.
% \end{itemize}
% \end{theorem}

% The authors of \cite{woodruff2022high} use a simple greedy algorithm to witness Theorem \ref{thm:subspace_sketching}. To analyze this algorithm, they bound the sum of \emph{online ridge leverage scores}.

% In the remainder of this section, we recover a result similar to that of Theorem \ref{thm:subspace_sketching} using the update rule from Algorithm \ref{alg:greedy_maxev}. 

\begin{theorem}
\label{thm:online_coreset_symmetric}
\nnote{main result}
\end{theorem}

We break the proof of Theorem \ref{thm:online_coreset_symmetric} into two parts.

\subsubsection{Part 1 -- Fully online symmetric ellipsoidal approximation algorithm}

The main result of this subsection is Lemma \ref{lemma:online_coreset_symmetric_ellipsoid}.

\begin{lemma}
\label{lemma:online_coreset_symmetric_ellipsoid}
Let $R_i$, $r_i$ be the smallest and largest values, respectively, that satisfy
\begin{align*}
    r_i \cdot \inparen{B_2^d \cap \mathsf{span}(\vx_1,\dots,\vx_i)} \subseteq \mathsf{conv}(\inbraces{\pm \vx_1,\dots,\pm\vx_i}) \subseteq R_i \cdot B_2^d.
\end{align*}
There exists an algorithm that, when given points $\vx_1,\dots,\vx_n$ one at a time in a stream, maintains an ellipsoid $\cE_i$ such that for all $i \in [n]$, we have
\begin{align*}
    \frac{1}{O\inparen{\sqrt{d\logv{\max_{i' \le i} \nfrac{R_{i'}}{r_{i'}}}}}} \cdot \inparen{\cE_i \cap \mathsf{span}(\vx_1,\dots,\vx_i)} \subseteq \mathsf{conv}(\inbraces{\pm \vx_1,\dots,\pm\vx_i}) \subseteq \inparen{\cE_i \cap \mathsf{span}(\vx_1,\dots,\vx_i)}.
\end{align*}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lemma:online_coreset_symmetric_ellipsoid}]
We reduce to a setting where we can apply Algorithm 2 due to \citet{mmo22}. Notice that Algorithm 2 requires an estimate $\xi$ for which $\xi \ge \nfrac{R}{r}$. It is easy to see that for all $i$ that $\nfrac{R_i}{r_i} \ge \nfrac{R}{r}$. 

We now show that by setting $\xi = \max_{i \le n} \nfrac{R_i}{r_i}$, Algorithm 2 does not perform any ``singular value inflation steps'', which means that we can apply it in a fully online manner. This easily follows from the below observation, which holds for all $i \in [n]$.
\begin{align*}
    \vx_i \cdot \nfrac{r_i}{R_i} \subseteq \mathsf{conv}\inparen{\pm \vx_1,\dots\pm \vx_i}
\end{align*}
This concludes the proof of Lemma \ref{lemma:online_coreset_symmetric_ellipsoid}.
\end{proof}

\subsubsection{Part 2 -- Reducing vertex selection to ellipsoidal approximations}

We now show how to convert \textit{any} fully online ellipsoidal approximation algorithm to one that returns a subset of vertices yielding an approximation to the original convex body. \nnote{should be reworded eventually} See Algorithm \ref{alg:subspace_sketching}.

\begin{algorithm}
\caption{Streaming $\linf$ Subspace Sketching\label{alg:subspace_sketching}}
\begin{algorithmic}[1]
    \State \textbf{Input}: A stream of points $\vx_1, \dots, \vx_n$, access to $\cU(\cE, \vx)$, the update rule for some fully online ellipsoidal approximation algorithm with state $\cE$ and input $\vx$.
    \State \textbf{Output}: Subset $S \subseteq [n]$ of size $O\inparen{d\logv{\max_{i \le n} \nfrac{R_i}{r_i}}}$ for which 
    \begin{align*}
        X\vert_S \subseteq X \subseteq O\inparen{\sqrt{\max_{i \le n} d\logv{d\cdot\nfrac{R_i}{r_i}+1}}} \cdot X\vert_S.
    \end{align*}
    \State Initialize $S = \emptyset$.
    \For{$t = 1, \ldots, n$}
        \State Read point $\vx_t$ from the stream.
        \State Let $d' = \mathsf{dim}(\mathsf{span}(\vx_1,\dots,\vx_{t-1}))$.
        \State Let $\cE_{t}' = \cU(\cE_{t-1}, \vx_t)$.
        \If{$\vx_t \notin \mathsf{span}(\vx_1,\dots,\vx_{t-1})$ or $\mathsf{Vol}_{d'}(\cE_t') \ge e \cdot \mathsf{Vol}_{d'}(\cE_{t-1})$}
            \State Let $\cE_t = \cE_{t'}$.
            \State Update $S$: $S \gets S \cup \inbraces{t}$.
        \Else
            \State Let $\cE_t = \cE_{t-1}$.
        \EndIf
    \EndFor
    \State \textbf{Output}: $S$.
\end{algorithmic}
\end{algorithm}

In Lemma \ref{lemma:online_coreset_symmetric_selection}, we show how Algorithm \ref{alg:subspace_sketching} gives the desired result.

\begin{lemma}
\label{lemma:online_coreset_symmetric_selection}
\nnote{lemma statement}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lemma:online_coreset_symmetric_selection}]
We first prove that $\abs{S}$ is small. Let $\lambda_{1,t},\dots,\lambda_{d,t}$ denote the semiaxes of $\cE_t$ (even though $\cE_t$ might not be fully dimensional, this will not affect this part of the analysis). Since $r_t \cdot B_2^d \subseteq \mathsf{conv}\inparen{\inbraces{\pm \vx_1, \dots, \pm \vx_t}} \subseteq R_t \cdot B_2^d$, we know that
\begin{align*}
    r_t^d \le \prod_{i=1}^d \lambda_{i,t} \le R_t^d.
\end{align*}
Since every point we add to $S$ increases $\prod_{i=1}^d \lambda_{i,t}$ by a factor of at least $e$, we must have for all $t \le n$ that
\begin{align*}
    \abs{S} \le \logv{\frac{R_t^d}{r_t^d}} \le d\logv{\frac{R_t}{r_t}}.
\end{align*}

Next, we show that our subset does provide a good approximation to $\mathsf{conv}\inparen{\inbraces{\pm \vx_1,\dots, \pm \vx_n}}$. Let $\cE_n$ be the state ellipsoid after Algorithm \ref{alg:subspace_sketching} has seen all $n$ points and observe that
\begin{align*}
    \mathsf{conv}\inparen{\inbraces{\pm \vx_1, \dots, \pm \vx_n}} \subseteq e \cdot \cE_n.
\end{align*}
Let $\alpha(\cU, \mX)$ be the approximation factor obtained by running the update rule $\cU$ on the stream of points $\mX = \inbraces{\vx_1,\dots,\vx_n}$ and notice that
\begin{align*}
    \frac{1}{\alpha(\cU, \mX\vert_S)} \cdot \cE_n &\subseteq \mathsf{conv}\inparen{\inbraces{\pm \vx_1, \dots, \pm \vx_n}} \subseteq e \cdot \cE_n \\
    \frac{1}{\alpha(\cU, \mX\vert_S)} \cdot \cE_n &\subseteq \mathsf{conv}\inparen{\inbraces{\pm \vx_i \text{ for } i \in S}} \subseteq \cE_n
\end{align*}
from which it follows that
\begin{align*}
    \frac{1}{e \cdot \alpha(\cU, \mX\vert_S)} \cdot \mathsf{conv}\inparen{\inbraces{\pm \vx_1, \dots, \pm \vx_n}} \subseteq \mathsf{conv}\inparen{\inbraces{\pm \vx_i \text{ for } i \in S}} \subseteq \mathsf{conv}\inparen{\inbraces{\pm \vx_1, \dots, \pm \vx_n}}.
\end{align*}

\nnote{Conclude with this for the general reduction, then give the below as a specific instantiation}

It remains to relate $e \cdot \alpha(\cU, \mX\vert_S)$ to $\alpha(\cU, \mX)$. Let $\kappaol(\mX)$ denote $\max_{i \le n} \nfrac{R_i}{r_i}$ and observe that
\begin{align*}
    \kappaol(\mX\vert_S) \le \alpha(\cU, \mX\vert_S) \cdot \kappaol(\mX) = e \cdot O\inparen{\sqrt{d\logv{\kappaol(\mX\vert_S)}}} \cdot \kappaol(\mX).
\end{align*}
After solving for $\kappaol(\mX\vert_S)$ and plugging this in, we have
\begin{align*}
    \alpha(\cU, \mX\vert_S) = O\inparen{\sqrt{d\logv{d\kappaol(\mX)}}}.
\end{align*}
This concludes the proof of Lemma \ref{lemma:online_coreset_symmetric_selection}. We remark that the extra $\sqrt{\log d}$ dependence is essentially subsumed by $\sqrt{\log\kappaol(\mX)}$ when $n = \mathsf{poly}(d)$ (see Lemma \ref{lemma:aspect_ratio_vs_n}).
\end{proof}

% Algorithm \ref{alg:subspace_sketching} yields Theorem \ref{thm:subspace_sketching_ours}.

% \begin{theorem}
% \label{thm:subspace_sketching_ours}
% Let $X \in \R^{n\times d}$ be presented in one pass over a row arrival stream. There is an algorithm $\cA$ which maintains a coreset $S \subseteq [n]$ such that:
% \begin{align*}
%     \text{for all } y \in \R^d, \maxnorm{X\vert_S \cdot y} \le \maxnorm{Xy} \le \alpha \cdot \maxnorm{X\vert_S \cdot y}
% \end{align*}
% where in the online coreset model, $\alpha = O\inparen{\sqrt{d\logv{d\cdot\nfrac{R}{r}+1}}}$ and $\abs{S} \le O\inparen{d \logv{d\cdot\nfrac{R}{r}+1}}$.
% \end{theorem}
% \begin{proof}
% We first prove Lemma \ref{lemma:cvx_hull_coreset}.

% \begin{lemma}
% \label{lemma:cvx_hull_coreset}
% The output $S$ of Algorithm \ref{alg:subspace_sketching} satisfies the following properties:
% \begin{itemize}
%     \item $S$ consists of at most $O\inparen{d\logv{\nfrac{R}{r}+1}}$ elements.
%     \item $X\vert_S \subseteq X \subseteq O\inparen{\sqrt{d\logv{\nfrac{R}{r}+1}}} \cdot X\vert_S$.
% \end{itemize}
% \end{lemma}
% \begin{proof}
% For notational simplicity, write $s \coloneqq d\logv{\nfrac{R}{r}}$.

% Observe that when we add elements to $S$, the volume of the state ellipsoid increases by a factor of at least $e$ in each iteration. Hence, over $\abs{S}$ iterations, we have:
% \begin{align*}
%     \frac{\mathsf{Vol}_d(\cE_n)}{\mathsf{Vol}_d(\cE_1)} \ge e^{\abs{S}}
% \end{align*}
% To get an upper bound on the left hand side, we prove the following claim.
% \begin{claim}
% For some constant $C$, in Algorithm \ref{alg:general_greedy_maxev}, we have:
% \begin{align*}
%     \frac{\mathsf{Vol}_d(\cE_n)}{\mathsf{Vol}_d(\cE_1)}\le C^{\nfrac{d}{2}}\cdot\logv{\xi+1}^{\nfrac{d}{2}} \cdot \xi^d \cdot \inparen{\frac{\max_{i\in[n]} \norm{x_i}}{\min_{i\in[n]} \norm{x_i}}}^d
% \end{align*}
% \end{claim}
% \begin{proof}
% Let $\astar = \nfrac{1}{R} \cdot I$. Observe that this is a valid choice of $\astar$ as used in the proofs of Theorems \ref{thm:simple_alg_arb_ellipsoid} and \ref{thm:greedy_approx}. Recall that we show that the $n$th iterate of Algorithm \ref{alg:general_greedy_maxev} satisfies, for some constant $C$:
% \begin{align*}
%     \fnorm{\astar\cdot A_n^{-1}}^2 = \sum_{i=1}^d \sigma_{i,n}^2 \le Cd\logv{\xi+1}
% \end{align*}
% By the AM-GM inequality, we have:
% \begin{align*}
%     \detv{\astar\cdot A_{n}^{-1}}^{\nfrac{2}{d}} = \inparen{\prod_{i=1}^d \sigma_{i,n}^2}^{\nfrac{1}{d}} \le \frac{\fnorm{\astar\cdot A_n^{-1}}^2}{d} = \frac{\sum_{i=1}^d \sigma_{i,n}^2}{d} \le C\logv{\xi+1}
% \end{align*}
% Furthermore, recall that our first iterate in Algorithm \ref{alg:general_greedy_maxev} satisfies:
% \begin{align*}
%     \detv{\astar\cdot A_{1}^{-1}} = \detv{\astar} \cdot \detv{A_{1}^{-1}} &= \frac{1}{R^d} \cdot \frac{\norm{x_1}^d}{\xi^{d-1}} \\
%     &\ge \frac{1}{R^d} \cdot \inparen{\frac{\min_{i \in [n]} \norm{x_i}}{\xi}}^d \\
%     &= \inparen{\frac{\min_{i\in[n]} \norm{x_i}}{\max_{i\in[n]} \norm{x_i}}}^d \cdot \frac{1}{\xi^d}
% \end{align*}
% We now write:
% \begin{align*}
%     \frac{\mathsf{Vol}_d(\cE_n)}{\mathsf{Vol}_d(\cE_1)} = \frac{\detv{A_n^{-1}}}{\detv{A_1^{-1}}} = \frac{\detv{\astar\cdot A_{n}^{-1}}}{\detv{\astar\cdot A_{1}^{-1}}} \le C^{\nfrac{d}{2}}\cdot\logv{\xi+1}^{\nfrac{d}{2}} \cdot \xi^d \cdot \inparen{\frac{\max_{i\in[n]} \norm{x_i}}{\min_{i\in[n]} \norm{x_i}}}^d
% \end{align*}
% \end{proof}
% Putting everything together gives:
% \begin{align*}
%     e^{\abs{S}} \le \frac{\mathsf{Vol}_d(\cE_n)}{\mathsf{Vol}_d(\cE_1)}\le C^{\nfrac{d}{2}}\cdot\logv{\xi+1}^{\nfrac{d}{2}} \cdot \xi^d \cdot \inparen{\frac{\max_{i\in[n]} \norm{x_i}}{\min_{i\in[n]} \norm{x_i}}}^d
% \end{align*}
% which implies:
% \begin{align*}
%     \abs{S} &\le \frac{d}{2}\log C + \frac{d}{2}\log\logv{\xi+1} + d\logv{\xi} + d\logv{\frac{\max_{i\in[n]} \norm{x_i}}{\min_{i\in[n]} \norm{x_i}}}\\
%     &\lesssim d\logv{\xi+1}+d\logv{\frac{\max_{i\in[n]} \norm{x_i}}{\min_{i\in[n]} \norm{x_i}}}
% \end{align*}
% as desired.

% We now focus on proving $X \subseteq O\inparen{\sqrt{s}} \cdot X\vert_S$.

% Notice that for all $i \in S$, we have $\norm{x_i} \ge r$ (since we initialize $\cE_0 = r\cdot B_2^d$). Hence, we have $\nfrac{r}{\sqrt{d}}\cdot B_2^d \subseteq X\vert_S$. It follows that $\nfrac{r}{\sqrt{d}}$ is a valid initialization for Algorithm \ref{alg:greedy_maxev} on the subset $e \cdot S$. Therefore, the output of Algorithm \ref{alg:greedy_maxev} on $e \cdot S$, which we will denote as $\cE_S$, satisfies:
% \begin{align*}
%     \frac{\cE_S}{O\inparen{\sqrt{d\logv{d\cdot\nfrac{R}{r}+1}}}} \subseteq e \cdot X\vert_S \subseteq \cE_S
% \end{align*}
% Next, observe that we only run the update rule for Algorithm \ref{alg:greedy_maxev} on the scaled elements in $S$ when we run Algorithm \ref{alg:subspace_sketching}. This is equivalent to running Algorithm \ref{alg:greedy_maxev} on the scaled elements in $S$, and since we initialize Algorithm \ref{alg:subspace_sketching} to $\cE_0 = \nfrac{r}{\sqrt{d}} \cdot B_2^d$, we have that $\cE_S$ is the final state ellipsoid of Algorithm \ref{alg:general_greedy_maxev}. This yields:
% \begin{align*}
%     X \subseteq \cE_S
% \end{align*}
% Putting our inclusions together gives:
% \begin{align*}
%     \frac{X}{O\inparen{\sqrt{d\logv{d\cdot\nfrac{R}{r}+1}}}} \subseteq \frac{\cE_S}{O\inparen{\sqrt{d\logv{d\cdot\nfrac{R}{r}+1}}}} \subseteq e \cdot X\vert_S
% \end{align*}
% In the end, we write:
% \begin{align*}
%     \frac{X}{O\inparen{\sqrt{d\logv{d\cdot\nfrac{R}{r}+1}}}} \subseteq e \cdot X\vert_S \subseteq X
% \end{align*}
% which is enough, as the factor of $e$ gets absorbed into the big-$O$ notation.
% \end{proof}

% We now show how Algorithm \ref{alg:subspace_sketching} and Lemma \ref{lemma:cvx_hull_coreset} together imply Theorem \ref{thm:subspace_sketching_ours}. Define:
% \begin{align*}
%     K\vert_S \coloneqq \inbraces{y \in \R^d \suchthat \maxnorm{X\vert_S\cdot y} \le 1}
% \end{align*}
% By the argument from Appendix \ref{section:mvie} we have:
% \begin{align*}
%     K\vert_S \subseteq K\vert_{[n]} \subseteq O\inparen{\sqrt{d\logv{d\cdot\nfrac{R}{r}+1}}}\cdot K\vert_S
% \end{align*}
% This is equivalent to:
% \begin{align*}
%     \text{for all } y \in \R^d, \maxnorm{X\vert_S \cdot y} \le \maxnorm{Xy} \le O\inparen{\sqrt{d\logv{d\cdot\nfrac{R}{r}+1}}} \cdot \maxnorm{X\vert_S \cdot y}
% \end{align*}
% as desired.
% \end{proof}

==> scratch.tex <==
% We first show the following intermediate result.
% \begin{lemma}
% For any sequence of inputs to Algorithm \ref{alg:greedy_maxev_noinit} $x_1,\dots,x_n$, let $T$ denote any subsequence for which for all $i \in [n] \setminus T$, $x_i$ does not cause Algorithm \ref{alg:greedy_maxev_noinit} to update its state ellipsoid (i.e., $x_i \in \cE_{i-1}$). Then, Theorem \ref{thm:simple_alg_approx} holds for $\conv{X\vert_T}$:
% \begin{align*}
%     \frac{\cE_n}{C\sqrt{d\logv{\kappaolconv{X}+1}}} \subseteq \conv{X\vert_T} \subseteq \cE_n
% \end{align*}
% \end{lemma}
% \begin{proof}
% Consider some $i \in [n]$ such that $i \notin T$. Observe that Algorithm \ref{alg:greedy_maxev_noinit} does not make an update upon seeing $x_i$, which means that $x_i \in \cE_{i-1}$. Since Algorithm \ref{alg:greedy_maxev_noinit} is monotone, we have that $x_i \in \cE_j$ for all $j \ge i-1$.

% From this, it follows that the following three sequences of length $n$ result in the same output ellipsoid $\cE_n$ from Algorithm \ref{alg:greedy_maxev_noinit}:
% \begin{align*}
%     X &= x_1, x_2, \dots, x_n \\
%     X\vert_T &= x_{t_1},\dots,x_{t_{\abs{T}}} \\
%     \widehat{X} &= x_{t_1},\dots,x_{t_{\abs{T}}},x_{i_{1}},\dots,x_{i_{n-\abs{T}}} \text{ for any ordering } i_j \text{ of the elements of } [n] \setminus T
% \end{align*}
% By Theorem \ref{thm:simple_alg_approx}, we know that:
% \begin{align*}
%     \frac{\cE_n}{C\sqrt{d\logv{\kappaolconv{X\vert_T}+1}}} &\subseteq \conv{X} \subseteq \cE_n \\
%     \frac{\cE_n}{C\sqrt{d\logv{\kappaolconv{X\vert_T}+1}}} &\subseteq \conv{X\vert_T} \subseteq \cE_n
% \end{align*}
% Putting these together gives us:
% \begin{align*}
%     \frac{\conv{X}}{C\sqrt{d\logv{\kappaolconv{X\vert_T}+1}}} \subseteq \frac{\cE_n}{C\sqrt{d\logv{\kappaolconv{X\vert_T}+1}}} \subseteq \conv{X\vert_T}
% \end{align*}
% Since $\conv{X} = \conv{\widehat{X}}$, we also know that:
% \begin{align*}
%     \frac{\cE_n}{C\sqrt{d\logv{\kappaolconv{\widehat{X}}+1}}} \subseteq \conv{\widehat{X}} \subseteq \cE_n
% \end{align*}
% Furthermore, it is easy to see that $\kappaolconv{X\vert_T} \le \kappaolconv{\widehat{X}}$.
% \end{proof}

==> update_step_old.tex <==
\section{Update Step - Details (to refactor)}
Consider a coordinate system where the previous ellipsoid is the unit ball centered at the origin, and the next point received is \(v = (1+s) \cdot e_1\). We can assume that \(s > 0\), as otherwise no update occurs. Let the previous ratio of inner to outer ellipsoid be \(\alpha\).
Further, let \(z^2 = x_2^2 + \ldots + x_d^2\) refer to the coordinates except \(x_1\).
The previous outer ellipsoid is defined by the equation \(x_1^2 + z^2 = 1\), and the inner ellipsoid is defined by \(x_1^2 + z^2 = \alpha^2\).

The current outer ellipsoid \(c + \cE'\) can be defined by \(A (x_1 - c)^2 + B z^2 = 1\) for \(A, B, c > 0\), with the corresponding inner ellipsoid as \(A (x_1 - c)^2 + B z^2 = \alpha'^2\) for current ratio \(\alpha'\), as shown in \Cref{fig:update_step}.
We will determine the largest value for \(\alpha'\) such that there exists a valid update with ratio \(\alpha'\).
A key observation is that this setup can be faithfully described by a two-dimensional picture: every dimension \(x_2\) through \(x_d\) behaves the same due to symmetry.


\begin{figure}[h]
\centering
\includegraphics[height=5cm]{update_step.png}
\caption{The update step.}
\label{fig:update_step}
\end{figure}

We first consider the equations that constrain the outer ellipsoid. \(\cE\) and \(c + \cE'\) must be tangent at some point, as otherwise \(\alpha'\) can be improved. Let \(\varphi \in [0, \pi/2]\) be the angle between the \(z\)-axis and the point of tangency of \(\cE\) and \(c + \cE'\), as shown in \Cref{fig:update_step_outer}.

\begin{figure}[h]
\centering
\includegraphics[height=5cm]{update_step_outer.png}
\caption{The outer ellipsoids in the update step.}
\label{fig:update_step_outer}
\end{figure}

Observe that at the point of tangency \((x, z) = (- \sin \varphi, \cos \varphi)\), the vector \((- \sin \varphi, \cos \varphi)\) defining the line \((x, z)\) is on and the gradient \((2A (x - c), 2Bz)\) of the equation defining the ellipsoid \(c + \cE'\) must be parallel. 
Thus \(B z x = A z(x-c)\), i.e.
\begin{equation}\label{eqn:outer_1}
    A (\sin \varphi + c) = B \sin \varphi
\end{equation}
As the point of tangency must be on \(c + \cE'\), we also have
\begin{equation}\label{eqn:outer_2}
    A (\sin \varphi + c)^2 + B \cos^2 \varphi = 1
\end{equation}
Finally, \((1+s, 0)\) must be on \(c + \cE'\) as well, so
\begin{equation}\label{eqn:outer_3}
    A (1+s - c)^2 = 1
\end{equation}

Solving these equations (\ref{eqn:outer_1}), (\ref{eqn:outer_2}), (\ref{eqn:outer_3}) for \(A, B, c\) in terms of \(s\) and \(\varphi\), we get:
% Older equations
% \begin{equation}
%     A = \frac{1}{\left(\Delta t-\frac{2 (-1 + {\Delta t}^2) \sin(\varphi)}{3 + 4 \Delta t \sin(\varphi) - \cos(2\varphi)}\right)^2}, \quad
%     B = \frac{3 + 4 \Delta t \sin(\varphi) - \cos(2\varphi)}{2 (1 + \Delta t \sin(\varphi))^2}, \quad
%     c = \frac{2 (-1 + {\Delta t}^2) \sin(\varphi)}{3 + 4 \Delta t \sin(\varphi) - \cos(2\varphi)}
% \end{equation}
\begin{equation}\label{eqn:outer_params}
\left.\begin{aligned}
    A = A^0(s, \varphi) &\defeq \frac{(\cos^2(\varphi)+2\sin(\varphi)(1+s + \sin(\varphi))^2}{(1+s + \sin(\varphi))^2(1+(1+s) \sin(\varphi))^2} \\
    B = B^0(s, \varphi) &\defeq \frac{1 + \sin^2(\varphi) + 2(1+s) \sin(\varphi)}{(1+(1+s) \sin(\varphi))^2}\\
    c = c^0(s, \varphi) &\defeq \frac{s(2+s)\sin(\varphi)}{1 + \sin^2(\varphi) + 2(1+s) \sin(\varphi)}
\end{aligned}\qquad
\right\}
\end{equation}
In summary, this gives a formula for the update \(c + \cE'\) in terms of \(s\) and \(\varphi\).
However, we have not yet considered how \(\alpha'\) is constrained.

Thus, we consider the equations that constrain the inner ellipsoid.
Let \(L\) be the line tangent to the previous inner ellipsoid \(\alpha \cE\) that goes through \(v\),
and let \((\hat{x}, \hat{z})\) be the point of tangency between \(L\) and \(\alpha \cE\).
Let \((x', z')\) be the point on \(c + \alpha' \cE'\) where the tangent line is parallel to \(L\).
This is illustrated in \Cref{fig:update_step_inner}.

\begin{figure}[h]
\centering
\includegraphics[height=5cm]{update_step_inner.png}
\caption{The inner ellipsoids in the update step.}
\label{fig:update_step_inner}
\end{figure}

We determine the equation defining \(L\). As the normal vector of \(L\) is parallel to \((\hat{x}, \hat{z})\), we can write it as \(\hat{x} x + \hat{z} z = \alpha^2\).
As \(v\) lies on \(L\), we have \(\hat{x} (1+s) = \alpha^2\) so \(\hat{x} = \frac{\alpha^2}{1+s}\).
Because \(\hat{x}^2 + \hat{z}^2 = \alpha^2\), we have \(\hat{z} = \sqrt{\alpha^2 - \frac{\alpha^4}{(1+s)^2}} = \alpha \sqrt{1 - \frac{\alpha^2}{(1+s)^2}}\).
By dividing all sides by \(\alpha^2\), we can also write the equation of \(L\) as \(\frac{x}{1+s} + z \sqrt{\frac{1}{\alpha^2} - \frac{1}{(1+s)^2}} = 1\).

The length of the major semi-axis (along \(x_1\)) of the current outer ellipsoid \(c + \cE'\) is \(1/\sqrt{A}\) by definition, so the length of the same axis of the inner ellipsoid is \(\alpha'/\sqrt{A}\).
As the leftmost point of \(c + \alpha' \cE'\) must be contained within \(\alpha \cE\), and it lies on the same axis as \((-\alpha, 0)\), we must have
\(c - \frac{\alpha'}{\sqrt{A}} \geq -\alpha\), so
\begin{equation}\label{eqn:inner_approx_1}
   \alpha' \leq \alpha^1(s, \varphi, \alpha) \defeq (\alpha + c) \sqrt{A}
\end{equation}

\((x', z')\) is defined by being on the inner ellipsoid, with its tangent parallel to \(L\).
The gradient of the equation defining \(c + \alpha' \cE'\) at \((x', z')\) is \((2 A (x' - c), 2 B z')\), which means
we have
\begin{equation}\label{eqn:inner_conv_1}
    A (x' - c) \sqrt{\frac{1}{\alpha^2}-\frac{1}{(1+s)^2}} = \frac{1}{1+s} B z'
\end{equation}
Because \((x', z')\) lies on the inner ellipsoid \(c + \alpha' \cE'\), we have
\begin{equation}\label{eqn:inner_conv_2}
    A (x' - c)^2 + B z'^2 = \alpha'^2
\end{equation}
Finally, \(c+ \alpha' \cE'\) must be contained within \(\conv{\alpha \cE \cup \{v\}}\), which implies that \((x', z')\) must be at least as close to the origin as \(L\). This gives
\begin{equation}\label{eqn:inner_conv_3}
    \frac{x'}{(1+s)} + \sqrt{\frac{1}{\alpha^2} - \frac{1}{(1+s)^2}} \cdot z' \leq 1
\end{equation}

The equation (\ref{eqn:inner_approx_1}) gives an upper bound on \(\alpha'\) using the leftmost point of \(\conv{\alpha \cE \cup \{v\}}\), so now we use (\ref{eqn:inner_conv_1}), (\ref{eqn:inner_conv_2}), (\ref{eqn:inner_conv_3}) to give another upper bound on \(\alpha'\) using \(L\).
Consider the smallest \(\alpha''\) such that \(c + \alpha'' \cE'\) touches \(L\), clearly \(\alpha'' \geq \alpha'\). If we define \((x', z')\) to lie on this ellipsoid \(c + \alpha'' \cE'\) instead, then (\ref{eqn:inner_conv_1}) is unchanged, (\ref{eqn:inner_conv_3}) becomes an equality,
and for (\ref{eqn:inner_conv_2}) we get \(\alpha''= A (x' - c)^2 + B z'^2 \geq \alpha'^2\).
The advantage of this rewrite is that now (\ref{eqn:inner_conv_1}) and (\ref{eqn:inner_conv_3}) form a linear system in \((x', z')\).
Solving this linear system, we get
\[
x' = \frac{(s+1) \left(A c (s+1) \sqrt{1-\frac{\alpha ^2}{(s+1)^2}} \sqrt{\frac{1}{\alpha ^2}-\frac{1}{s+1}}+\alpha  B\right)}{A (s+1)^2 \sqrt{1-\frac{\alpha ^2}{(s+1)^2}} \sqrt{\frac{1}{\alpha ^2}-\frac{1}{s+1}}+\alpha  B}, \quad
z' = \frac{\alpha  A (s+1) (-c+s+1) \sqrt{\frac{1}{\alpha ^2}-\frac{1}{s+1}}}{A (s+1)^2 \sqrt{1-\frac{\alpha ^2}{(s+1)^2}} \sqrt{\frac{1}{\alpha ^2}-\frac{1}{s+1}}+\alpha  B}
\]

Using this solution in (\ref{eqn:inner_conv_2}), we get our second upper bound on \(\alpha'\) in addition to (\ref{eqn:inner_approx_1}):
\begin{equation}\label{eqn:inner_approx_2}
    \alpha' \leq \alpha^2(s, \varphi, \alpha) \defeq \sqrt{\frac{A B (-c+s+1)^2 \left(A (s+1) \left(-\alpha ^2+s+1\right)+\alpha ^2 B\right)}{\left(A (s+1)^2 \sqrt{1-\frac{\alpha ^2}{(s+1)^2}} \sqrt{\frac{1}{\alpha ^2}-\frac{1}{s+1}}+\alpha  B\right)^2}}
\end{equation}

Thus the best possible \(\alpha'\) is the minimum of these two upper bounds:
\begin{equation}\label{eqn:inner_approx_param}
    \alpha^{0}(s, \varphi, \alpha) \defeq \min(\alpha^1(s, \varphi, \alpha), \alpha^2(s, \varphi, \alpha))
\end{equation}

